WaterSeeker: Pioneering Efficient Detection of Watermarked Segments in Large Documents

Watermarking algorithms for large language models (LLMs) have attained high accuracy in detecting LLM-generated text. However, existing methods primarily focus on distinguishing fully watermarked text from non-watermarked text, overlooking real-world scenarios where LLMs generate only small sections within large documents. In this scenario, balancing time complexity and detection performance poses significant challenges. This paper presents WaterSeeker, a novel approach to efficiently detect and locate watermarked segments amid extensive natural text. It first applies an efficient anomaly extraction method to preliminarily locate suspicious watermarked regions. Following this, it conducts a local traversal and performs full-text detection for more precise verification. Theoretical analysis and experimental results demonstrate that WaterSeeker achieves a superior balance between detection accuracy and computational efficiency. Moreover, its localization capability lays the foundation for building interpretable AI detection systems. Our code is available at https://github.com/THU-BPM/WaterSeeker.

==> table/ratio_2000.tex <==
\begin{table*}[t]
\caption{Comparison of WaterSeeker with other baselines under the mixing ratio of 4.8\%-16.7\%. 
}
\centering
\tiny
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{cccccc|cccc}
\toprule
 \multirow{2}{*}{Model}& \multirow{2}{*}{Method} & \multicolumn{4}{c}{KGW} & \multicolumn{4}{c}{Aar} \\
\cmidrule{3-10}
& & FPR $\downarrow$ & FNR $\downarrow$ & F1 $\uparrow$ & IoU $\uparrow$ & FPR $\downarrow$ & FNR $\downarrow$ & F1 $\uparrow$ & IoU $\uparrow$ \\
\midrule
\multirow{7}{*}{Llama-2-7b} & Full-text Detection & 0.000 & 1.000 \color{red}[0.967]\color{black} & 0.000 \color{red}[0.065]\color{black} & 0.005 &  0.000 & 1.000 \color{red}[0.873]\color{black} & 0.000 \color{red}[0.225]\color{black} & 0.018  \\
& WinMax & 0.003 & 0.257 & 0.851 & 0.669 & 0.003 & 0.413 & 0.738 & 0.533  \\
& FLSW-100 & 0.000 & 0.473 & 0.690 & 0.440 & 0.003 & 0.570 & 0.600 & 0.350\\
& FLSW-200 & 0.000 & 0.420 & 0.734 & 0.446 & 0.000 & 0.607 & 0.565 & 0.327 \\
& FLSW-300 & 0.003 & 0.630 & 0.539 & 0.339 & 0.000 & 0.777 & 0.365 & 0.257 \\
& FLSW-400 & 0.003 & 0.850 & 0.260 & 0.246 & 0.000 & 0.883 & 0.209 & 0.200 \\
& \cellcolor{gray!25}  WaterSeeker(Ours) & \cellcolor{gray!25}0.003 & \cellcolor{gray!25}0.287 & \cellcolor{gray!25}0.831 & \cellcolor{gray!25}0.642 & \cellcolor{gray!25}0.003 & \cellcolor{gray!25}0.443 & \cellcolor{gray!25}0.714 & \cellcolor{gray!25}0.501 \\
\midrule
\multirow{7}{*}{Mistral-7b} & Full-text Detection & 0.000 & 1.000 \color{red}[0.980]\color{black} & 0.000  \color{red}[0.039]\color{black} & 0.003 & 0.000 & 1.000 \color{red}[0.870]\color{black} & 0.000 \color{red}[0.230]\color{black} & 0.017 \\
& WinMax & 0.000 & 0.220 & 0.876 & 0.710 & 0.003 & 0.353 & 0.783 & 0.590 \\
& FLSW-100 & 0.000 & 0.470 & 0.693 & 0.447 & 0.000 & 0.487 & 0.678 & 0.415  \\
& FLSW-200 & 0.000 & 0.360 & 0.780 & 0.497 & 0.003 & 0.500 & 0.665 & 0.371  \\
& FLSW-300 & 0.000 & 0.533 & 0.636 & 0.386 & 0.003 & 0.760 & 0.386 & 0.285  \\
& FLSW-400 & 0.000 & 0.747 & 0.404 & 0.288 & 0.003 & 0.887 & 0.203 & 0.212   \\
& \cellcolor{gray!25}  WaterSeeker(Ours) & \cellcolor{gray!25}0.000 & \cellcolor{gray!25}0.227 & \cellcolor{gray!25}0.872 & \cellcolor{gray!25}0.701 & \cellcolor{gray!25}0.003  & \cellcolor{gray!25}0.363 &\cellcolor{gray!25}0.776 & \cellcolor{gray!25}0.574  \\
\bottomrule
\end{tabular}
}
\label{tab:ratio_2000}
\end{table*}

==> table/ratio_500.tex <==
\begin{table*}[t]
\caption{Comparison of WaterSeeker with other baselines under the mixing ratio of 16.7\%-44.4\%. 
}
\centering
\tiny
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{cccccc|cccc}
\toprule
 \multirow{2}{*}{Model}& \multirow{2}{*}{Method} & \multicolumn{4}{c}{KGW} & \multicolumn{4}{c}{Aar} \\
\cmidrule{3-10}
& & FPR $\downarrow$ & FNR $\downarrow$ & F1 $\uparrow$ & IoU $\uparrow$ & FPR $\downarrow$ & FNR $\downarrow$ & F1 $\uparrow$ & IoU $\uparrow$ \\
\midrule
\multirow{7}{*}{Llama-2-7b} & Full-text Detection & 0.000 & 1.000 \color{red}[0.787]\color{black} & 0.000 \color{red}[0.352]\color{black} & 0.081 & 0.000 & 1.000 \color{red}[0.693]\color{black} & 0.000 \color{red}[0.469]\color{black} & 0.109 \\
& WinMax & 0.000 & 0.247 & 0.859 & 0.685 & 0.000 & 0.373 & 0.770 & 0.568 \\
& FLSW-100 & 0.000 & 0.470 & 0.693 & 0.445 & 0.000 & 0.557 & 0.614 & 0.380 \\
& FLSW-200 & 0.000 & 0.383 & 0.763 & 0.461 & 0.000 & 0.553 & 0.618 & 0.340 \\
& FLSW-300 & 0.000 & 0.553 & 0.618 & 0.360 & 0.000 & 0.690 & 0.473 & 0.298 \\
& FLSW-400 & 0.000 & 0.740 & 0.413 & 0.265 & 0.000 & 0.837 & 0.281 & 0.231 \\
& \cellcolor{gray!25}  WaterSeeker(Ours) & \cellcolor{gray!25}0.000 & \cellcolor{gray!25}0.277 & \cellcolor{gray!25}0.839 & \cellcolor{gray!25}0.647 & \cellcolor{gray!25}0.000 & \cellcolor{gray!25}0.410 & \cellcolor{gray!25}0.742 & \cellcolor{gray!25}0.522 \\
\midrule
\multirow{7}{*}{Mistral-7b} & Full-text Detection & 0.000 & 1.000 \color{red}[0.847]\color{black} & 0.000 \color{red}[0.266]\color{black} & 0.061 & 0.000 & 1.000 \color{red}[0.697]\color{black} &  0.000 \color{red}[0.465]\color{black} & 0.112 \\
& WinMax & 0.000 & 0.270 & 0.844 & 0.652 & 0.000 & 0.350 & 0.788 & 0.588 \\
& FLSW-100 & 0.000 & 0.510 & 0.658 & 0.432 & 0.000 & 0.530 & 0.639 & 0.393 \\
& FLSW-200 & 0.000 & 0.407 & 0.745 & 0.442  & 0.000 & 0.510 & 0.658 & 0.369 \\
& FLSW-300 & 0.000 & 0.570 & 0.601 & 0.352 & 0.000 & 0.690 & 0.473 & 0.294\\
& FLSW-400 & 0.000 & 0.760 & 0.387 & 0.243 & 0.000 & 0.827 & 0.295 & 0.246 \\
& \cellcolor{gray!25}  WaterSeeker(Ours) & \cellcolor{gray!25}0.000  & \cellcolor{gray!25}0.303 &\cellcolor{gray!25}0.821 & \cellcolor{gray!25}0.612 & \cellcolor{gray!25}0.000 & \cellcolor{gray!25}0.407 & \cellcolor{gray!25}0.745 & \cellcolor{gray!25}0.543 \\
\bottomrule
\end{tabular}
}
\label{tab:ratio_500}
\end{table*}

==> table/ratio_5000.tex <==
\begin{table*}[t]
\caption{Comparison of WaterSeeker with other baselines under the mixing ratio of 2\%-7.4\%. 
}
\centering
\tiny
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{cccccc|cccc}
\toprule
 \multirow{2}{*}{Model}& \multirow{2}{*}{Method} & \multicolumn{4}{c}{KGW} & \multicolumn{4}{c}{Aar} \\
\cmidrule{3-10}
& & FPR $\downarrow$ & FNR $\downarrow$ & F1 $\uparrow$ & IoU $\uparrow$ & FPR $\downarrow$ & FNR $\downarrow$ & F1 $\uparrow$ & IoU $\uparrow$ \\
\midrule
\multirow{7}{*}{Llama-2-7b} & Full-text Detection & 0.000 & 1.000 \color{red}[0.990]\color{black} &  0.000 \color{red}[0.020]\color{black} & 0.001 & 0.000 & 1.000 \color{red}[0.957]\color{black} & 0.000 \color{red}[0.083]\color{black} & 0.002 \\
& WinMax & 0.003 & 0.317 & 0.810 & 0.621 & 0.010 & 0.380 & 0.761 & 0.565\\
& FLSW-100 & 0.000 & 0.520 & 0.649 & 0.413 & 0.003 & 0.523 & 0.644 & 0.375 \\
& FLSW-200 & 0.000 & 0.457 & 0.704 & 0.404 & 0.000 & 0.560 & 0.611 & 0.350 \\
& FLSW-300 & 0.003 & 0.663 & 0.502 & 0.297 & 0.000 & 0.767 & 0.378 & 0.283 \\
& FLSW-400 & 0.003 & 0.867 & 0.235 & 0.230 & 0.000 & 0.920 & 0.148 & 0.205 \\
& \cellcolor{gray!25}  WaterSeeker(Ours) & \cellcolor{gray!25}0.003 & \cellcolor{gray!25}0.357 & \cellcolor{gray!25}0.781 & \cellcolor{gray!25}0.570 & \cellcolor{gray!25}0.010 & \cellcolor{gray!25}0.407 & \cellcolor{gray!25}0.740 & \cellcolor{gray!25}0.536 \\
\midrule
\multirow{7}{*}{Mistral-7b} & Full-text Detection & 0.000 & 1.000 \color{red}[0.990]\color{black} & 0.000  \color{red}[0.020]\color{black} & 0.000 & 0.000 & 1.000 \color{red}[0.937]\color{black} & 0.000 \color{red}[0.119]\color{black} & 0.004 \\
& WinMax & 0.003 & 0.227 & 0.871 & 0.700 & 0.010 & 0.370 & 0.768 & 0.570 \\
& FLSW-100 & 0.000 & 0.503 & 0.664 &  0.443 & 0.000 & 0.543 & 0.627 & 0.364\\
& FLSW-200 & 0.000 & 0.350 & 0.788 &  0.497 & 0.003 & 0.540 & 0.629 & 0.362\\
& FLSW-300 & 0.000 & 0.527 & 0.643 & 0.392 & 0.003 & 0.763 & 0.382 & 0.269 \\
& FLSW-400 & 0.000 & 0.783 & 0.357 & 0.281 & 0.003 & 0.910 & 0.165 & 0.203 \\
& \cellcolor{gray!25}  WaterSeeker(Ours) & \cellcolor{gray!25}0.000  & \cellcolor{gray!25}0.243 &\cellcolor{gray!25}0.861 & \cellcolor{gray!25}0.676 & \cellcolor{gray!25}0.010 & \cellcolor{gray!25}0.383 & \cellcolor{gray!25}0.758& \cellcolor{gray!25}0.548 \\
\bottomrule
\end{tabular}
}
\label{tab:ratio_5000}
\end{table*}

==> table/robustness.tex <==
\begin{table}[htbp]
    \caption{}
    \centering
    \begin{tabular}{lccc}
        \toprule
        \textbf{Dataset} & \textbf{FPR$\downarrow$} & \textbf{FNR$\downarrow$} & \textbf{F1$\uparrow$} \\
        \midrule
        KGW-Llama & 0.000 & 0.983 & 0.033 \\
        KGW-Mistral & 0.000 & 0.993 & 0.013\\
        Aar-Llama & 0.000 & 0.980 & 0.039 \\
        Aar-Mistral & 0.000 & 0.980 & 0.039 \\
        \bottomrule
    \end{tabular}
    \label{tab:full_text}
\end{table}

==> table/time.tex <==
\begin{table*}[t]
    \caption{Average detection time per sample for various detection methods ($N \approx 10,000$, Unit: s).}
    \centering
    {\small
    \resizebox{0.98\textwidth}{!}{
        \renewcommand{\arraystretch}{1.2} 
        \begin{tabular}{cccccccc}
        \hline
             & Full-text Detection & WinMax & FLSW-100 & FLSW-200 & FLSW-300 & FLSW-400& WaterSeeker  \\\hline
            KGW & 1.70 & 14.16 & 1.76 & 1.76 & 1.79 & 1.80 & 1.75 \\
            Aar & 0.54 & 2733.78 & 1.62 & 1.65 & 1.66 & 1.64 & 1.68 \\\hline
        \end{tabular}
    }
    }
    \label{tab:time}
\end{table*}
